Automating Human Tutor-Style Programming Feedback: Leveraging GPT-4 Tutor Model for Hint Generation and GPT-3.5 Student Model for Hint Validation

Generative AI and large language models hold great promise in enhancing programming education by automatically generating individualized feedback for students. We investigate the role of generative AI models in providing human tutor-style programming hints to help students resolve errors in their buggy programs. Recent works have benchmarked state-of-the-art models for various feedback generation scenarios; however, their overall quality is still inferior to human tutors and not yet ready for real-world deployment. In this paper, we seek to push the limits of generative AI models toward providing high-quality programming hints and develop a novel technique, GPT4Hints-GPT3.5Val. As a first step, our technique leverages GPT-4 as a ``tutor'' model to generate hints -- it boosts the generative quality by using symbolic information of failing test cases and fixes in prompts. As a next step, our technique leverages GPT-3.5, a weaker model, as a ``student'' model to further validate the hint quality -- it performs an automatic quality validation by simulating the potential utility of providing this feedback. We show the efficacy of our technique via extensive evaluation using three real-world datasets of Python programs covering a variety of concepts ranging from basic algorithms to regular expressions and data analysis using pandas library.

==> figs/illustration_regex_p144/content_obfuscated/testcase.tex <==
Your Code's output is: \textcolor{InputOutput}{[('Benjamin', 'Davis'), ('William', 'Clark'), ('Elias', 'Jovanovic'), ('Hakim', 'Botros'), ('Emilie', 'Lorentsen'), ('Jake', 'Wood'), ('Fatemeh', 'Akhtar'), ('Kim', 'Weston'), ('Yasmin', 'Dar'), ('Viswamitra', 'Upandhye'), ('Killian', 'Kaufman'), ('Elwood', 'Page'), ('Elodie', 'Booker'), ('Adnan', 'Chen'), ('Hank', 'Spinka'), ('Hannah', 'Bayer')]}
It's Correct output is: \textcolor{InputOutput}{['Benjamin Davis',  'William Clark',  'Elias Jovanovic',  'Hakim Botros',  'Emilie Lorentsen',  'Jake Wood',  'Fatemeh Akhtar',  'Kim Weston',  'Yasmin Dar',  'Viswamitra Upandhye',  'Killian Kaufman',  'Elwood Page',  'Elodie Booker',  'Adnan Chen',  'Hank Spinka',  'Hannah Bayer']}
